Faithful Interpretation for Graph Neural Networks

Currently, attention mechanisms have garnered increasing attention in Graph Neural Networks (GNNs), such as Graph Attention Networks (GATs) and Graph Transformers (GTs). It is not only due to the commendable boost in performance they offer but also its capacity to provide a more lucid rationale for model behaviors, which are often viewed as inscrutable. However, Attention-based GNNs have demonstrated instability in interpretability when subjected to various sources of perturbations during both training and testing phases, including factors like additional edges or nodes. In this paper, we propose a solution to this problem by introducing a novel notion called Faithful Graph Attention-based Interpretation (FGAI). In particular, FGAI has four crucial properties regarding stability and sensitivity to interpretation and final output distribution. Built upon this notion, we propose an efficient methodology for obtaining FGAI, which can be viewed as an ad hoc modification to the canonical Attention-based GNNs. To validate our proposed solution, we introduce two novel metrics tailored for graph interpretation assessment. Experimental results demonstrate that FGAI exhibits superior stability and preserves the interpretability of attention under various forms of perturbations and randomness, which makes FGAI a more faithful and reliable explanation tool.

==> table/fig3.tex <==
\begin{figure}[htbp] 
    \setlength{\tabcolsep}{1pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{center}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cc}
    % Coauthor-Physics & Coauthor-CS \\
    \includegraphics[width=0.49\linewidth]{figure/GAT_coauthor_phy_vanilla_topK.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/GAT_pubmed_vanilla_topK.pdf} \\
    \includegraphics[width=0.49\linewidth]{figure/GAT_coauthor_phy_FGAI_topK.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/GAT_pubmed_FGAI_topK.pdf}
    \end{tabular*}
    \caption{Visualizations of the attention results for both the vanilla model (GAT) and FGAI before and after perturbation.
    % showcasing top-$k$ important neighboring nodes and edges from a specific node before and after perturbation. 
    The red color connects the nodes appeared in top-$k$ nodes.
    }
    \label{fig:vis2}
    \end{center}
\vspace{-15pt}
\end{figure}


==> table/fig4.tex <==
% \begin{figure*}[t] 
%     \setlength{\tabcolsep}{1pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1.0} % Default value: 1
%     \begin{center}
%     \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccc}
%      Amazon-cs & Amazon-photo & Coauthor & Pubmed \\
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_amazon-cs_1.pdf} &
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_amazon-photo_1.pdf} &
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_coauthor-phy_1.pdf} &
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_pubmed_1.pdf} \\
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_amazon-cs_2.pdf} &
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_amazon-photo_2.pdf} &
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_coauthor-phy_2.pdf} &
%     \includegraphics[width=0.245\linewidth]{figure/line_chart_pubmed_2.pdf}
%     \end{tabular*}
%     \caption{Positive perturbation and negative perturbation results for both the vanilla model (GAT) and FGAI on the four datasets. We calculate the accuracy by removing the important features for positive perturbations while removing the unimportant features for negative perturbations.}
%     \label{fig:inter}
%     \end{center}
% \vspace{-0.2in}
% \end{figure*}

\begin{figure}[htbp] 
    \setlength{\tabcolsep}{1pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{center}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cc}
    Amazon-cs & Amazon-photo \\
    \includegraphics[width=0.49\linewidth]{figure/line_chart_amazon-cs_1_attacked.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/line_chart_amazon-photo_1_attacked.pdf} \\
    \includegraphics[width=0.49\linewidth]{figure/line_chart_amazon-cs_2_attacked.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/line_chart_amazon-photo_2_attacked.pdf}
    \end{tabular*}
    \caption{Positive perturbation and negative perturbation results for both the vanilla model (GAT) and FGAI. We calculate the accuracy by removing the important features for positive perturbations while removing the unimportant features for negative perturbations.}
    \label{fig:inter_app}
    \end{center}
\vspace{-0.2in}
\end{figure}


==> table/fig4_1.tex <==
\begin{figure}[htbp] 
    \setlength{\tabcolsep}{1pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.0} % Default value: 1
    \begin{center}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cc}
     Coauthor & Pubmed \\
    \includegraphics[width=0.49\linewidth]{figure/line_chart_coauthor-phy_1_attacked.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/line_chart_pubmed_1_attacked.pdf} \\
    \includegraphics[width=0.49\linewidth]{figure/line_chart_coauthor-phy_2_attacked.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/line_chart_pubmed_2_attacked.pdf}
    \end{tabular*}
    \caption{Positive perturbation and negative perturbation results for both the vanilla model (GAT) and FGAI. We calculate the accuracy by removing the important features for positive perturbations while removing the unimportant features for negative perturbations.}
    \label{fig:inter}
    \end{center}

\end{figure}



==> table/fig5.tex <==
\begin{figure}[htbp] 
    \setlength{\tabcolsep}{1pt} % Default value: 6pt
    \renewcommand{\arraystretch}{0.8} % Default value: 1
    \begin{center}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cc}
     Amazon-photo & Amazon-cs  \\
    \includegraphics[width=0.49\linewidth]{figure/bar_chart_Amazon-photo.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/bar_chart_Amazon-cs.pdf} \\
    Coauthor & Pubmed \\
    \includegraphics[width=0.49\linewidth]{figure/bar_chart_Coauthor.pdf} &
    \includegraphics[width=0.49\linewidth]{figure/bar_chart_Pubmed.pdf}
    \end{tabular*}
    \caption{Results of micro-averaged F1 scores for various models before and after perturbation considering both the vanilla approach and the FGAI method.}
    \label{fig:stab}
    \end{center}

\end{figure}


==> table/loss_2.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{figure/loss_components_amazon_photo_FGAI_GAT.pdf}
    \caption{The illustration showing the training loss decreasing with increasing epochs for the GAT model applying FGAI on the Amazon-Photo dataset. \label{fig:loss2}}
\end{figure}

==> table/loss_3.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{figure/loss_components_obgn_arxiv_GATv2.pdf}
    \caption{The illustration showing the training loss decreasing with increasing epochs for the GATv2 model applying FGAI on the ogbn-Arxiv dataset. \label{fig:loss3}}
\end{figure}

==> table/loss_4.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{figure/loss_components_obgn_arxiv_GAT.pdf}
    \caption{The illustration showing the training loss decreasing with increasing epochs for the GAT model applying FGAI on the ogbn-Arxiv dataset. \label{fig:loss4}}
\end{figure}

==> table/tab3.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.0}
\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{cccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}  
& \multirow{2}{*}{\textbf{Model}} 

& \multicolumn{2}{c}{\textbf{Amazon-photo}} 
& \multicolumn{2}{c}{\textbf{Amazon-cs}} 
& \multicolumn{2}{c}{\textbf{Coauthor}} 
& \multicolumn{2}{c}{\textbf{Pubmed}} 
& \multicolumn{2}{c}{\textbf{ogbn-arxiv}} \\ 

\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12} & 

& \textbf{$F_{slope}^{-}\downarrow$} & \textbf{$F_{slope}^{+}\uparrow$} 
& \textbf{$F_{slope}^{-}$} & \textbf{$F_{slope}^{+}$} 
& \textbf{$F_{slope}^{-}$} & \textbf{$F_{slope}^{+}$} 
& \textbf{$F_{slope}^{-}$} & \textbf{$F_{slope}^{+}$} 
& \textbf{$F_{slope}^{-}$} & \textbf{$F_{slope}^{+}$} \\ 

\midrule

\multirow{5}{*}{\textbf{Vanilla}} 
& GAT & 1.1598 & 1.0059 
      & 0.8098 & 0.3273 
      & 0.0014 & 0.5746 
      & 0.0894 & 0.5983 
      & 1.0436 & 0.9066 \\
& GAT+LN & 0.5505 & 0.1393 
         & 0.4566 & 0.2657 
         & 0.0009 & 0.0005 
         & 0.0705 & 0.5360 
         & 0.6544 & 0.8301 \\
& GAT+AT & 1.3837 & 0.4326 
         & 0.9411 & 0.6024 
         & 0.0016 & 0.8391 
         & 0.0639 & 0.3974
         & 0.9946 & 1.0558 \\
& GATv2 & 1.2514 & 0.8248
        & 0.7838 & 0.1041
        & 0.0018 & 0.5432
        & 0.0770 & 0.6653 
        & 0.8784 & 1.0934 \\
% & ProGNN & 0 & 0
%          & 0 & 0 
%          & 0 & 0 
%          & 0 & 0 \\

\midrule
\midrule

\multirow{5}{*}{\textbf{FGAI}} 
& GAT & 1.0998 & 0.6216
        & 0.7316 & 0.2223
        & 0.0020 & 0.8774
        & 0.0527 & 0.7579 
        & 1.0853 & 1.0886 \\
& GAT+LN & 1.0224 & 0.2615 
         & 0.4137 & 0.1850 
         & 0.0014 & 0.7144 
         & 0.0528 & 0.3818 
         & 0.8612 & 0.7813 \\
& GAT+AT & 0.8924 & 0.5408 
         & 0.9917 & 0.4569 
         & 0.0028 & 0.8655 
         & 0.0663 & 0.5759 
         & 0.5241 & 0.7506 \\
& GATv2 & 1.2361 & 0.6307 
         & 0.5146 & 0.0413 
         & 0.0030 & 0.7012 
         & 0.0587 & 0.7633 
         & 0.7851 & 0.8538 \\
% & ProGNN & 0 & 0
%          & 0 & 0 
%          & 0 & 0 
%          & 0 & 0 \\

\bottomrule
\end{tabular}
}
\caption{Results of micro-averaged F1 scores for various models before and after perturbation considering both the vanilla approach and the FGAI method.}
\label{tab:1.1}
\end{table*}

